High-frequency wave power observed in the solar chromosphere with IBIS and ALMA

We present observational constraints on the solar chromospheric heating contribution from acoustic waves with frequencies between 5 and 50 mHz. We utilize observations from the Dunn Solar Telescope in New Mexico complemented with observations from the Atacama Large Millimeter Array collected on 2017 April 23. The properties of the power spectra of the various quantities are derived from the spectral lines of Ca II 854.2 nm, H I 656.3 nm, and the millimeter continuum at 1.25 mm and 3 mm. At the observed frequencies the diagnostics almost all show a power law behavior, whose particulars (slope, peak and white noise floors) are correlated with the type of solar feature (internetwork, network, plage). In order to disentangle the vertical versus transverse plasma motions we examine two different fields of view; one near disk center and the other close to the limb. To infer the acoustic flux in the middle chromosphere, we compare our observations with synthetic observables from the time-dependent radiative hydrodynamic RADYN code. Our findings show that acoustic waves carry up to about 1 kW m$^{-2}$ of energy flux in the middle chromosphere, which is not enough to maintain the quiet chromosphere, contrary to previous publications.

==> Sections/Bibliography.tex <==
\begin{thebibliography}{}
\bibitem[Alissandrakis(1981)]{PFFFS} Alissandrakis, C.~E.\ 1981, \aap, 100, 197
\bibitem[Aschwanden(2005)]{2005psci.book.....A} Aschwanden, M.~J.\ 2005, Springer, New York, Berlin
\bibitem[Biermann(1948)]{1948ZA.....25..161B} Biermann, L.\ 1948, \zap, 25, 161
\bibitem[Bogod \& Gelfreikh(1980)]{1980SoPh...67...29B} Bogod, V.~M., \& Gelfreikh, G.~B.\ 1980, \solphys, 67, 29
\bibitem[Cauzzi et al.(2008)]{Cauzzi_2008} Cauzzi, G., Reardon, K.~P., Uitenbroek, H., et al.\ 2008, \aap, 480, 515
\bibitem[Cavallini(2006)]{Cavallini2006}Cavallini, F. 2006, \solphys, 236, 415
\bibitem[Cranmer \& Woolsey(2015)]{2015ApJ...812...71C} Cranmer, S.~R., \& Woolsey, L.~N.\ 2015, \apj, 812, 71
\bibitem[Cranmer et al.(2017)]{Solar_wind_review} Cranmer, S.~R., Gibson, S.~E., \& Riley, P.\ 2017, \ssr, 212, 1345
\bibitem[Carlsson \& Stein(1997)]{Carlsson_and_Stein} Carlsson, M., \& Stein, R.~F.\ 1997, \apj, 481, 500
\bibitem[Culhane et al.(2007)]{EIS_ref} Culhane, J.~L., Harra, L.~K., James, A.~M., et al.\ 2007, \solphys, 243, 19
\bibitem[Cuntz et al.(2007)]{2007ApJ...657L..57C} Cuntz, M., Rammacher, W., \& Musielak, Z.~E.\ 2007, \apjl, 657, L57i
\bibitem[de Wijn et al.(2005)]{de_Wijn_High_freq} de Wijn, A.~G., Rutten, R.~J., \& Tarbell, T.~D.\ 2005, \aap, 430, 1119
\bibitem[De Moortel \& Browning(2015)]{Coronal_Heating_3} De Moortel, I., \& Browning, P.\ 2015, Philosophical Transactions of the Royal Society of London Series A, 373, 20140269
\bibitem[De Pontieu et al.(2014)]{IRIS} De Pontieu, B. et al., 2014, \solphys, 289, 2733-2779
\bibitem[Deng et al.(2015)]{MFGS_info} Deng, H., Zhang, D., Wang, T., et al.\ 2015, \solphys, 290, 1479
\bibitem[Dunn(1964)]{Dunn_1} Dunn, R.~B.\ 1964, \ao, 3, 1353
\bibitem[Dunn \& Smartt(1991)]{Dunn_2} Dunn, R.~B., \& Smartt, R.~N.\ 1991, Advances in Space Research, 11, 139
\bibitem[Evans et al.(1963)]{Evans_power} Evans, J.~W., Michard, R., \& Servajean, R.\ 1963, Annales d'Astrophysique, 26, 368
\bibitem[Fleck \& Deubner(1989)]{Fleck1989} Fleck, B., \& Deubner, F.-L.\ 1989, \aap, 224, 245
\bibitem[Fleck et al.(2010)]{Fleck2010} Fleck, B., Straus, T., Carlsson, M., et al.\ 2010, Bulletin of the American Astronomical Society, 41, 403.09
\bibitem[Fleck \& von der L{\"u}he(2017)]{Fleck2017} Fleck, B., \& von der L{\"u}he, O.\ 2017, \solphys, 292, 178
\bibitem[Fontenla et al.(1993)]{Fontenla1993} Fontenla, J.~M., Avrett, E.~H., \& Loeser, R.\ 1993, \apj, 406, 319
\bibitem[Fontenla et al.(2011)]{Fontenla2011} Fontenla, J. M., et al., 2011, J. Geophys. Res., 116, D20108
\bibitem[Fossum \& Carlsson(2006)]{Fossum_and_Carlsson} Fossum, A., \& Carlsson, M.\ 2006, \apj, 646, 579
\bibitem[Grant et al.(2018)]{Alfvenic_waves_heat_penumbra} Grant, S. T., Jess, D., Zaqarashvili, T., Beck, C., et al.\ 2018, Nature Physics, 14, 480–483
\bibitem[Grebinskij et al.(2000)]{2000A&AS..144..169G} Grebinskij, A., Bogod, V., Gelfreikh, G., et al.\ 2000, \aaps, 144, 169
\bibitem[Groth(1975)]{Groth1975} Groth, E.~J.\ 1975, \apjs, 29, 285
\bibitem[Gudiksen et al.(2011)]{BIFROST} Gudiksen, B.~V., Carlsson, M., Hansteen, V.~H., et al.\ 2011, \aap, 531, A154
\bibitem[Hansteen et al.(2000)]{Hansteen_HF_waves} Hansteen, V.~H., Betta, R., \& Carlsson, M.\ 2000, \aap, 360, 742
\bibitem[Hoyng(1976)]{Hoyng1976}Hoyng, P. 1976, \aap, 47, 449-452
\bibitem[Jaeggli et al.(2010)]{Jaeggli2010} Jaeggli, S.A., Lin, H., Mickey, D.L., et al., 2010, MmSAI, 81, 763
\bibitem[Jess et al.(2010)]{Jess2010} Jess, D.B., Mathioudakis, M., Christian, D.J., et al, 2010, \solphys, 261, 363.
\bibitem[Jing et al.(2011)]{Jing_fibrils} Jing, J., Yuan, Y., Reardon, K., et al.\ 2011, \apj, 739, 67
\bibitem[Judge(2006)]{Chromosphere_review} Judge, P.\ 2006, in ASP Conf.\ Ser.\ 354,  NSO Workshop, Sacramento Peak, Sunspot \ Eds.  J. Leibacher, R. F. Stein, and H. Uitenbroek. San Francisco: Astronomical Society of the Pacific, 2006., p.259
\bibitem[Koutchmy et al.(1983)]{Koutchmy_waves} Koutchmy, S., Zhugzhda, I.~D., \& Locans, V.\ 1983, \aap, 120, 185
\bibitem[Keller \& Solis Team(2001)]{SOLIS} Keller, C.~U., \& Solis Team, 2001, in Advanced Solar Polarimetry -- Theory, Observation, and Instrumentation -- 20TH NSO/Sac Summer Workshop, ASP Conf.\ Proc.\, 236, Eds. M. Sigwarth
\bibitem[Kosugi et al.(2007)]{Hinode_mission_overview} Kosugi, T., Matsuzaki, K., Sakao, T., et al.\ 2007, \solphys, 243, 3
\bibitem[Labeyrie(1970)]{Speckle} Labeyrie, A.\ 1970, \aap, 6, 85
\bibitem[Leenaarts et al.(2012)]{Leenaarts_H_alpha} Leenaarts, J. et al., 2012, \apj, 749, 136-150
\bibitem[Lemen et al.(2012)]{AIA} Lemen, J. R.,  A. M. Title et al., 2012, \solphys, 275, 17-40
\bibitem[Lites et al.(2007)]{2007MmSAI..78..148L} Lites, B., Casini, R., Garcia, J., \& Socas-Navarro, H.\ 2007, \memsai, 78, 148
\bibitem[Lites \& Ichimoto(2013)]{MERLIN_Code} Lites, B.~W., \& Ichimoto, K.\ 2013, \solphys, 283, 601
\bibitem[Mathioudakis et al.(2013)]{Alfven_wave_review} Mathioudakis, M., Jess, D.~B., \& Erd{\'e}lyi, R.\ 2013, \ssr, 175, 1
\bibitem[McMullin et al.(2007)]{CASA}McMullin, J. P., Waters, B., Schiebel, D., Young, W., Golap, K. \ 2007, Astronomical Data Analysis Software and Systems XVI (ASP Conf. Ser. 376), ed. R. A. Shaw, F. Hill, D. J. Bell (San Francisco, CA: ASP), 127
\bibitem[Molnar et al.(2018)]{Molnar_1} Molnar, M., Reardon, K., Chai, Y., Uitenbroek, H., Cauzzi, G., Gary, D., Cranmer, S., 2018, in prep.
\bibitem[November \& Simon(1988)]{LCT} November, L.~J., \& Simon, G.~W.\ 1988, \apj, 333, 427
\bibitem[Pesnell et al.(2012)]{HMI}	Pesnell, W.D et al. 2012, \solphys, 275, 3-15
\bibitem[Phillips et al.(2015)]{ALMA_1} Phillips, N., Hills, R., Bastian, T., et al.\ 2015, Revolution in Astronomy with ALMA: The Third Year, 499, 347
\bibitem[Puschmann et al.(2012)]{GFPI} Puschmann, K.~G., Denker, C., Kneer, F., et al.\ 2012, Astronomische Nachrichten, 333, 880
\bibitem[Reardon et al.(2008)]{Reardon_Turbulence} Reardon, K.~P., Lepreti, F., Carbone, V., \& Vecchio, A.\ 2008, \apjl, 683, L207
\bibitem[Rimmele(2004)]{AO_Rimmele} Rimmele, T.~R.\ 2004, \procspie, 5490, 34
\bibitem[Scharmer(2006)]{CRISP} Scharmer, G.~B.\ 2006, \aap, 447, 1111
\bibitem[Schou et al.(2012)]{SDO} Schou, J., P.H. Scherrer et al., 2012, \solphys, 275,  229-259
\bibitem[Schwarzschild(1948)]{1948ApJ...107....1S} Schwarzschild, M.\ 1948, \apj, 107, 1
\bibitem[Socas-Navarro \& Uitenbroek(2004)]{H_alpha_formation} Socas-Navarro, H., \& Uitenbroek, H.\ 2004, \apjl, 603, L129
\bibitem[Tsuneta et al.(2008)]{SOT_ref} Tsuneta, S., Ichimoto, K., Katsukawa, Y., et al.\ 2008, \solphys, 249, 167
\bibitem[Uitenbroek(2001)]{RH} Uitenbroek, H. 2001, \apj, 557, 389-398
\bibitem[Uitenbroek(2003)]{Uitenbroek2003} Uitenbroek, H.\ 2003, \apj, 592, 1225
\bibitem[Ulmschneider \& Musielak(2003)]{Chromospheric_heating_review} Ulmschneider, P., \& Musielak, Z.\ 2003, in Preparing for ATST, ASP Conf.\ Ser.\, 286, NSO Workshop, Sunspot, Eds. A. Pevtsov, H. Uitenbroek.
\bibitem[Wedemeyer-B{\"o}hm, \& Steffen(2007)]{2007A&A...462L..31W} Wedemeyer-B{\"o}hm, S., \& Steffen, M.\ 2007, \aap, 462, L31.
\bibitem[Wedemeyer et al.(2015)]{ALMA_ref}Wedemeyer, S. et al., 2015, \ssr, 200, 1-4, 1-73
\bibitem[Withbroe \& Noyes(1977)]{1977ARA&A..15..363W} Withbroe, G.~L., \& Noyes, R.~W.\ 1977, \araa, 15, 363
\bibitem[W{\"o}ger et al.(2008)]{Speckle_code} W{\"o}ger, F., von der L{\"u}he, O., \& Reardon, K.\ 2008, \aap, 488, 375.
\bibitem[Wunnenberg et al.(2002)]{Wunnenberg_waves} Wunnenberg, M., Kneer, F., \& Hirzberger, J.\ 2002, \aap, 395, L51.
\bibitem[van Noort et al.(2005)]{MOMFBD} van Noort, M., Rouppe van der Voort, L., \& L{\"o}fdahl, M.~G.\ 2005, \solphys, 228, 191 i

\end{thebibliography}


==> Sections/Excess_power.tex <==
\section{Excess power in the H$\alpha$ power spectra}
\label{sec:HF_bump}
	
The peak observed in some spectral properties derived from H$\alpha$ is ... 
it is similar to the high frequency bump observed in~\cite{2019NatAs.tmp..502J}
in \ion{He}{1} 10830~{\AA}.

\subsection{Systematic origins of the excess power are improbable}



\subsection{Correlations with the physical properties of the underlying properties}

==> Sections/Solar_explanation.tex <==
\section{Possible Solar explanations?} 
\label{sec:Solar_explanations}

After not finding any evidence of instrumental effects in Section~\ref{sec:Systematics} causing a periodic variation to the image, we will discuss several physical phenomena which could be
responsible for the excess power in the H$\alpha$ observations. 


\subsection{Propagation of waves}
\label{subsec:Prop_waves}
The Fourier transformation provides us with phase information, beside the amplitude information. The phases between the constituent functions provide us with information about the 
propagation characteristics of the waves with these frequencies. Furthermore, if we have two different diagnostics observed simultaneously, we can use their phase difference to estimate the 
propagation properties of the waves. If the two diagnostics whose phases we compare are separated in space we can estimate phase speed of the waves.

Figure~\ref{fig:phase_delay} shows a phase delay diagram between the measured H$\alpha$ COG velocity and the bisector velocity for the 17:11 UT time series. A phase delay diagram shows the phase difference of   
the different Fourier components of the two quantities of interest. Such plots are two dimensional histograms, where we plot along the x-axis frequency and along the y-axis phase difference. Since the
frequency is sampled regularly in a FFT, only the x-axis comprises of multiple 1-D histograms. If there is a phenomenon detected in both diagnostics which
has a stable phase relationship (or offset as a function of the period), then
we see a region of enhancement in the phase delay diagram. If no coherency is detected in the diagnostics, we no region of enhancement is detected in the phase delay diagram and the phases remain widely scattered. 

In this case we are interested to explore if there is any propagation signature between the two velocities (COG and bisector) in which the high-frequency 
excess power was detected. We see in Figure~\ref{fig:phase_delay} that there is significant coherency in the low frequencies around the 3-minute oscillations. An interesting observation is that 
there is no phase delay for the low frequency waves, which sheds doubt on the idea that different parts of the line sample different regions of the atmosphere. The 
coherency between the COG velocity and the bisector velocity is also pretty close to unity, which suggests that the two diagnostics are measuring the same 
velocity. Furthermore, this coherency 
disappears at higher frequencies, as previously 
pointed out by \cite{Fleck1989}. However, at 42 mHz -- the frequency of the excess power in this time series, typical for FOV2 -- we see an enhancement in the coherency of the signal as the phases cluster together. Furthermore, the phase difference in 
the region at 42 mHz is the same as the low frequency region. This might give us a clue about its origin - is it a wave driven from the photospheric convective overshoot or some sort of intensity leakage? 

\begin{figure}[h!]
  \includegraphics[width=0.5\textwidth]{Figures/Phase_delay_171115_COG_BIS.png}
  \caption{Phase delay diagram between H$\alpha$ COG velocity and the bisector velocity for the time series at 17:11 UT. The high values (yellow color) mean higher number of pixels having this phase
  delay between their COG velocity and bisector velocities. We see that at higher frequencies we don't have any coherent signals, as has been shown before. Curiously, we can see the coherent signal around 
  42 mHz which corresponds to the unexplained peak in the H$\alpha$ power spectrum.    
}
    \label{fig:phase_delay}
\end{figure}


\subsection{Resonant Alfv\'{e}n waves in low-lying closed loops}
\label{subsec:Resonant_Alfvenic_waves}

If the high-frequency signal is originating from a MHD wave, it has a signature of incompressible Alfv\'{e}n wave since we detect 
it only in Doppler displacements.
From Figure~\ref{fig:Where} we see that the signal is structured in narrow regions. Hence, we can model it as magnetic loops which act 
like 
resonant cavities. The period in this case is determined by the Alfv\'{e}n crossing time of these loops. In order to investigate more 
this possibility we need to retrieve the magnetic field topology from the SOTSP observations.

\label{subsec:PFFFS}
In order to recover the magnetic field topology in the region of interest we extrapolated the magnetic field from the boundary conditions 
provided from the photospheric observations of SOTSP. Even though the
extrapolations based on photospheric fields are not ideal for chromospheric studies, since the chromosphere is not force-free, 
for the quiet region of interest it is an acceptable approximation. Furthermore, for quiet sun
areas there is almost no twist in the magnetic field, which allows us to use as a suitable approximation a potential field extrapolation which satisfies the equation: 

\begin{equation}
\nabla \times \vec{B} = 0. 
\label{eqn:B_PFE}
\end{equation}

We used a publicly available code from M. K. Georgoulis(JHU/APL), based on \cite{PFFFS} that solves the boundary value problem based on the Fourier transforms. However, spectral methods have 
disadvantages, as the discretization of the domain if not properly expanded in the numerical setup of the problem can cause ringing. We used a single scan for both fields of view as input for the magnetic extrapolation 
as we did not want to average over multiple scans which would have smeared the fine magnetic structures. 

The extrapolated magnetic field model was then interpolated to the plate scale of IBIS and aligned to the far-wing of H$\alpha$. This step is required because the pointing precision of the spacecraft is on the order of 
arcseconds which corresponds to shifts of tens of pixels in terms of IBIS plate scale. The far H$\alpha$ wing is a suitable diagnostic to align magnetograms to, because the regions of high magnetic flux appear bright 
H$\alpha$ wing magnetograms.

After some previous work with RH \citep{RH} we \citep{Molnar_1} estimated that the height of formation of H$\alpha$ is about 1.5 Mm on average. Hence, we will use this value for the following estimates of the 
height of formation of the radiation in which we see the oscillatory power.

If the source of the unexpected peak in the power spectrum is due to Alfv\'{e}nic waves, we will expect to have a correlation between the inclination of the magnetic field and the Doppler velocity power due to projection 
effects. Alfv\'{e}nic waves are transverse in nature, creating velocity oscillations in the direction perpendicular to the direction of propagation. Hence, if we have a vertical flux tube observed from above 
we will not see any Doppler displacements or other typical imprints of Alfv\'{e}nic waves. If we have a horizontal flux tube observed from above, we will see the full amplitude of the propagating Alfv\'{e}nic wave as 
Doppler shift signature.

Figure~\ref{fig:inclination_vs_power} shows that there is no clear correlation between the excess power at 40 mHz and the field inclination derived from our extrapolation. 
This sheds some doubt on the Alfv\'{e}n wave
nature of the waves, but in general it is known that 
photospheric potential field extrapolations underestimate the horizontal magnetic fields in the chromosphere~\citep{Jing_fibrils}. Thus, there is a possibility that the noisy data from the SOTSP 
are not a suitable boundary condition for a meaningful chromospheric magnetic field extrapolation, which might underestimate
the horizontal magnetic fields. 

Figure~\ref{fig:b_strength_vs_power} shows the lack of correlation between the extrapolated magnetic field strength at the formation region of H$\alpha$ and the excess power there. This lack of correlation between the two
might suggest that a process not associated with the magnetic field permeating the solar atmosphere is responsible directly for the excess power.

\begin{figure}[h!]
  \includegraphics[width=0.5\textwidth]{Figures/Inclination_vs_power.png}
  \caption{COG velocity power at 40 mHz vs inclination of the magnetic field extrapolation at height 1.5Mm above the photosphere, where H$\alpha$ is formed. There is no correlation between inclined field lines and 
  excess power.}
    \label{fig:inclination_vs_power}
\end{figure}

\begin{figure}[h!]
  \includegraphics[width=0.5\textwidth]{Figures/B_field_magnitude_vs_power.png}
  \caption{COG velocity power at 40 mHz vs the magnetic field strength at height 1.5 Mm above the photosphere from the extrapolation. There is no correlation between the strength and 
  excess high-frequency power. }
    \label{fig:b_strength_vs_power}
\end{figure}



==> Sections/Systematics.tex <==
\section{Systematic effects, or just the real Sun}
\label{sec:Systematics}


The subtle nature of the detected signal requires us to examine its possible instrumental origin. In the following chapter we present an 
analysis of some possible instrumental sources of periodic disturbances as well as the possibility of periodic disturbances from the data processing.

\subsection{Instrumental effects}

The most probable instrumental disturbances that can introduce such a sharp peak in the power spectra of the data are associated with time varying components of the instrument. 
Since the filter wheel is not changing, the only 
moving components of the instrument are the Fabry P\'{e}rot etalons and the times of the exposures. If the Fabry-P\'{e}rot system is not stable and samples at different wavelength positions, this could introduce a 
possible time dependent wavelength shift in the data. On the other hand, if the exposures are not taken with normally distributed intervals, as assumed in our data reduction, this could also introduce periodic signal in our signal.

\subsubsection{Periodicity of the exposures}

IBIS was operated close to the limit of the memory buffer of the imaging cameras. Hence, there is a possibility that periodic irregular 
sampling was introduced from not having the randomly distributed time intervals
between exposures. Theoretically, this
could influence the power of the data (even though that the solar images will not change on the time scales of milliseconds at these resolutions).

We calculated the power spectrum of the deviation from the mean time interval between exposures, which is a measure of the irregularity of the time sampling. 
This quantity was derived by first calculating the average time step between exposures. Knowing this the expected exposure time was calculated and subtracted from the 
actual exposure realization. The result is presented in Fig.~\ref{fig:Shutter_periodicity} for both a series in which the high-frequency peak was detected    
(series H$\alpha$ 14:18 UT) and one in which there was no detection (Ca II 8542 17:04 UT). There is no characteristic excess power around the frequency region of interest (shaded in red).  
However, there are high-frequency peaks and their harmonics, which have their fundamental frequency around the 0.3 Hz (3 second) mark. These are most 
probably due to the small additional time delay that was introduced by the instrument control software between individual spectral scans. 
Therefore, we dismiss the possibility that the unexpected high-frequency signal was introduced through this 
mechanism.


\begin{figure}[h!]
  \includegraphics[width=0.5\textwidth]{Figures/Shutter_periodicity.png}
  \caption{The power spectrum of the deviations from regular temporal sampling. The green spectrum is from Ca II 17:04 UT time series with no detection of the excess high-frequency power;
  the blue power spectrum is from the H$\alpha$ 14:18 UT time series in which 
  we detected the unexpected high-frequency peak. The shaded in red area is the frequency domain where the excess high-frequency power is detected. There is no excess power in that frequency region in the 
  sampling irregularity, thus we reject the hypothesis that sampling aperiodicity introduces the excess power detected in the H$\alpha$ ``fast'' scans. The two power spectra were shifted along the y-axis with a constant
  for better readability of the graph.}
\label{fig:Shutter_periodicity}
\end{figure}


\subsubsection{Stability of the FP etalons}
Another systematic effect that has to be examined is the temporal stability of the Fabry-P\'{e}rot etalon system. 
If the two Fabry-P\'{e}rot etalons showed slight variations in their spectral tuning positions in successive scans this could result in different parts of the spectral line being imaged at the same nominal wavelength position.
The resulting irregular sampling of 
different intensities could result into a different intensity and introduce a systematic offset in the derived spectral properties. We note that a spectral shift of 
$\sim$2.5 m{\AA} (the spectral shift due to the unexpected high-frequency signal) corresponds to a shift in the cavity in the etalons of $\sim$8 {\AA}. It is important to note that
a shift like this would cause a global shift over the whole field 
of view, which is not what we see in Fig.\ref{fig:Where}. Furthermore, a disturbance of this sort will introduce a spurious signal in every scanned spectral line.

In Figure~\ref{fig:FP-stability} we show the power spectrum at every wavelength location (along the rows) averaged over the whole image. There is no excess power present in any of the 
wavelength positions in the frequency region of interest around 40 mHz in both the H$\alpha$ scan and the Ca II scan. Thus, we can conclude that there is no temporal disturbance in the Fabry-P\'{e}rot etalon system   
that produces such irregular sampling.

\begin{figure*}[ht!]
\subfigure[Scan in H$\alpha$ at 17:11 UT.]{
\label{fig:first}
  \includegraphics[width=\columnwidth]{Figures/fft_FP_stability_Ha.png}}
\qquad
\subfigure[Scan in Ca II 8542 at 17:04 UT.]{
\label{fig:second}
\includegraphics[width=\columnwidth]{Figures/fft_FP_stability_ca.png}}
\caption{Power in the intensity of single wavelength positions from the spectral line profiles used for calculating the velocities and the other spectral line properties described in the text. In the two panes there are 
  fast scans from two data sets, H$\alpha$ at 17:11 UT on the left, that does exhibit the extra power at around 40 mHz and a Ca II IR scan which does not exhibit excess power at higher frequencies. As we see there is no excess 
  power in the left pane around 40 mHz, which confirms the stability of the Fabry-P\'erot etalon filter system.}
  \label{fig:FP-stability}
\end{figure*}

\subsection{Residual seeing effects}

The other time dependent component of the data acquisition and processing is the seeing reduction. We have destretched IBIS to
HMI continuum images as reference in order to remove the bulk and subfield seeing motions   
in our images. However, this does not perfectly correct all the seeing distortions and might leave some seeing effects with periodic nature. Therefore, 
in the next subsections we will investigate the possible sources of 
seeing induced high-frequency power excess in H$\alpha$. 

\subsubsection{Bulk misalignment of the narrowband images}

The first step of the seeing reduction processing involves alignment of the white-light images to a HMI white-light, which acts like an absolute reference. Hence, a  
test of the quality of the bulk alignment of our data between consecutive images. This misalignment was measured through the minimum of the cross correlation between the two images with an IDL 
routine xyoff.pro, distributed in SolarSoft\footnote{\href{https://sohowww.nascom.nasa.gov/solarsoft/}{SolarSoft} is a free IDL library for solar physics.}. We used the same routine for initial calibration,
and the test of the alignment, but it has been robustly tested.
The images are aligned to
precision of less than a pixel, but still cross talk between pixels might be induced from the seeing, which will smear the signal over adjacent pixels. The power spectrum of the jitter was calculated and is presented in 
Figure~\ref{fig:power_xyoff_center}. There is no signal in the power spectrum of bulk jitter in the frequency region of interest, thus we can discard the hypothesis that the unexpected peak is caused by it.   

\begin{figure}[ht!]
  \includegraphics[width=0.5\textwidth]{Figures/Power_xyoff_center_image.png}
  \caption{The figure represents the power spectrum of the residual bulk displacements of several image sequences, represented with the different colors. The shaded region (in red) represents
  the region of the frequency domain where the excess power is detected. We do not see any signatures of misalignment of the images 
  in the frequency region of interest, hence we can discard the hypothesis that bulk misalignment of images
  introduce the periodic signal observed in H$\alpha$.}
 \label{fig:power_xyoff_center}
\end{figure}

\subsubsection{Residual seeing effects from the small box cross correlations}
\label{sec:Seeing_residuals}
The second step in the destretching procedure was the local correlation tracking~\citep{LCT}. Malfunctioning of this step could have resulted in small scale
uncorrelated image motion that would produce
cross talk between pixels. If this effect was causing the high-frequency excess of power in H$\alpha$ then we would see the most power in pixels close to the locations in the images where the most cross talk
can occur. The locations of the image most prone to cross talk are the sharp boundaries between structures, where the gradient of the measured quantity is greatest. 
If seeing induced high-frequency excess was the case, then the pixels with the highest high-frequency power are going to be associated with regions with the 
highest gradient in the measured intensity.

Figure~\ref{fig:grad_vel_vs_power} shows a 2D histogram of the gradient of the COG velocity in a image vs the average power between 38 mHz and 48 mHz for time series 15:18 UT. These frequencies are the region of the high-frequency power excess in FOV2.
The signal was detected in this time sequence
and we averaged over its physical extent.
The figure shows that the pixels with the highest power in this frequency range are not close to large gradients in the velocity -- even the opposite is seen. This supports the idea that 
seeing reduction procedure is not responsible for excess high-frequency power. Furthermore, even the opposite could be inferred from Figure~\ref{fig:grad_vel_vs_power} -- where there are large gradients, close to the 
boundaries of structures, the seeing induced cross talk between pixels reduces the amplitude of the high-frequency signals, as their coherency time is shorter than the longer time perturbations.

\begin{figure*}[ht!]
\subfigure[Gradient of COG Velocity against power around 44 mHz.]{
\label{fig:first_2}
  \includegraphics[width=\columnwidth]{Figures/Fig_gradient_image.png}}
\qquad
\subfigure[Gradient of line core intensity against power around 44 mHz.]{
\label{fig:second_2}
  \includegraphics[width=\columnwidth]{Figures/Fig_gradient_image_2.png}}
\caption{Histograms of the average power at the unexpected peak against the gradient of the image of the quantity that the power was derived from for the time series of 15:18UT. 
  In figure~\ref{fig:first_2} the COG velocity gradient is plotted against the excess power; in Figure~\ref{fig:second_2} the line core intensity gradient is plotted against the average power at the aforementioned 
  frequency region. We see that the regions with the highest excess of high-frequency power are close to regions with
  no gradients, which refutes the hypothesis of seeing induced cross talk origin of the unexpected signal.}
\label{fig:grad_vel_vs_power}
\end{figure*}

\subsubsection{Estimating seeing conditions and their periodicities}

Recurring deterioration of image quality on a certain timescale could produce excess power at a certain frequency as it will smear out the velocity signal in a periodic pattern. This could be 
introduced by the Adaptive Optics system as well, not only the atmospheric turbulence causing the ``seeing''.

We investigated this possibility by calculating a image quality metric for each image in the time sequence and sought out periodicities in the seeing metric.
The image quality metric of our choice is the Median Filtered 
Gradient Similarity (MFGS) \citep{MFGS_info}. MFGS compares the similarity between the absolute value of a gradient of the original image and value of the gradient 
for the same image
convolved with a median filter.
We chose MFGS over the regular RMS of the image, because MFGS has been proven to be more robust for images with 
high contrast regions like sunspots or pores on the border of the image. MFGS returns a value between 0 and 1, increasing for improving image quality. 

We calculated the MFGS with a simple Python script\footnote{\emph{mfgs.py} in the author's repository; see Page 21 for link.} for the white-light and narrowband images which exhibited the excessive high-frequency power  
and for ones which did not. Then we calculated the power spectrum of the time series of the MFGS values for these two series. The results are presented in Figure~\ref{fig:MFGS_PS}. The shaded in red frequency region is the domain where the excess power is observed - nothing significant is seen in that 
region, so we can discard the hypothesis that AO or some other periodic image deterioration causes the spike.  

\begin{figure}[ht!]
  \includegraphics[width=0.5\textwidth]{Figures/Power_MFGS}
  \caption{Power spectrum of the estimated MFGS for every frame in the different time series. We don't see a significant difference between the ones with or without detected excess power. The power spectra are shifted apart by a constant to improve the clarity of the figure.}
  \label{fig:MFGS_PS}
\end{figure}

